Elucidating coherent structures, transport barriers and entrainment in turbulent fountains in stratified media

We analyse the flow organization of turbulent fountains in stratified media under different conditions, using three-dimensional finite-time Lyapunov exponents. The dominant Lagrangian coherent structures responsible for the transport barriers in three different configurations suggest a self-similarity behaviour. After proposing a criterion for delimiting the boundary surface of the uprising fountain, we quantify the entrainment and re-entrainment rates under fully developed flow conditions using the proper coefficients. Finally, our analysis was applied to the Selective Inverted Sink, a technological application of turbulent fountains, identifying turbulence as the primary mechanism favouring the device's efficiency.

==> quotation.tex <==
%\todoq{Editar quotation.tex}

%\bf{Editar quotation.tex}

%The ``lead paragraph'' is encapsulated with the \LaTeX\ \verb+quotation+ environment and is formatted as a single paragraph before the first section heading. (The \verb+quotation+ environment reverts to its usual meaning after the first sectioning command.) Note that numbered references are allowed in the lead paragraph.
%
%The lead paragraph will only be found in an article being prepared for the journal \textit{Chaos}.
